Two New Methods for Counting and Tracking the Evolution of Polar Faculae

Polar faculae (PFe) are the footpoints of magnetic field lines near the Sun's poles that are seen as bright regions along the edges of granules. The time variation in the number of PFe has been shown to correlate with the strength of the polar magnetic field and to be a predictor of the subsequent solar cycle. Due to the small size and transient nature of these features, combined with different techniques and observational factors, previous counts of PFe differ in magnitude. Further, there were no scalable techniques to measure the statistical properties of faculae. Using data from the Helioseismic and Magnetic Imager (HMI) onboard the Solar Dynamics Observatory (SDO), we present two new methods for tracking faculae and measuring their properties. In the first, we calculate the standard deviation of the HMI images over one day, visualizing the faculae as streaks. The facular lifetime is found by dividing the angular streak length by the latitude-dependent rotation rate. We apply this method to 134 days of data over 11 years. The distribution of facular lifetimes has a mean of 6.0 hours, a FWHM of 5.4 hours, and a skew towards longer lifetimes, with some lasting up to 1 day. In the second method, we overlay images of the progressive standard deviation with the HMI magnetogram to show the close relationship between facular candidates and the magnetic field. The results allow us to distinguish between motion due to the Sun's rotation and "proper motion" due to faculae moving across the Sun's surface, confirming that PFe participate in convective motions at the poles. Counts of PFe using both methods agree with previous counts in their variation with the solar cycle and the polar magnetic field. These methods can be extended to automate the identification and measurement of other properties of of PFe, which would allow for daily measurements of all faculae since SDO began operation in 2010.

==> SOLA_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})


